Urban Street Network Design and Transport-Related Greenhouse Gas Emissions around the World

This study estimates the relationships between street network characteristics and transport-sector CO2 emissions across every urban area in the world and investigates whether they are the same across development levels and urban design paradigms. The prior literature has estimated relationships between street network design and transport emissions -- including greenhouse gases implicated in climate change -- primarily through case studies focusing on certain world regions or relatively small samples of cities, complicating generalizability and applicability for evidence-informed practice. Our worldwide study finds that straighter, more-connected, and less-overbuilt street networks are associated with lower transport emissions, all else equal. Importantly, these relationships vary across development levels and design paradigms -- yet most prior literature reports findings from urban areas that are outliers by global standards. Planners need a better empirical base for evidence-informed practice in under-studied regions, particularly the rapidly urbanizing Global South.

==> tables/table3.tex <==
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
      & \multicolumn{2}{c}{Least Developed Countries (LDC)} & \multicolumn{2}{c}{Less Developed Countries (LDCL)} & \multicolumn{2}{c}{Most Developed Countries (MDR)} \\
     \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7} & 
     \multicolumn{1}{c}{coef.}  & \multicolumn{1}{c}{beta} & \multicolumn{1}{c}{coef.} & \multicolumn{1}{c}{beta} & \multicolumn{1}{c}{coef.} & \multicolumn{1}{c}{beta} \\
\midrule
 K average (log) &  -4.352*** &  -0.593   & -1.408*** &  -0.069   &  -1.252*** & -0.034    \\
            & (1.155)  & & (0.464)  & & (0.376)  &  \\
			
 Straightness & -8.136 & -0.378 & -6.298*** &  -0.081 &  -1.839 &  0.889  \\
  & (4.848) & & (1.584) & & (1.462) &  \\
  
 Intersection density &  7.776 & 0.039 & -0.876 & -0.013 &  9.578 &  0.014  \\
 & (6.252) & & (3.207) & & (12.682) & \\
 
 Length per capita (log) &   1.025*** & 0.348 & 0.711*** & 0.322 & 0.115 & 0.132 \\
 & (0.274) & & (0.106) & & (0.175) & \\
 
 Built up area (log) &   0.363*** & 0.432 &  0.374*** & 0.437 &  0.158*** & 0.146  \\
    & (0.064) & & (0.029) & & (0.026) &  \\
	
 Open space (log) &  0.568 &  0.209  &  0.374*** & 0.072 &  0.376*** & 0.071 \\
    & (0.480) & & (0.165) & & (0.056) & \\
	
 Population density (log) &  -0.121 & -0.251 &  0.033 & 0.024 &   -0.801*** & -1.607  \\
       & (0.245) & & (0.119) & & (0.176) &  \\
	   
 GDP per capita (log) &   0.099 & 0.043 &  0.140** &  0.090 &  0.244*** & 0.328  \\
   & (0.084) & & (0.046) & & (0.053) &  \\
   
 Night light per capita (log) &   0.181*** & 0.043 &  0.266*** &  0.207   & 0.154** & 0.119  \\
& (0.031) & & (0.032) & & (0.052) & \\

 Grade median & -11.356 & -0.103 & -17.190*** &  -0.128 & 1.697 & 0.008  \\
  & (5.852) & & (2.419) & & (2.580) &  \\
\midrule
    $n$ &  735 &  &  5708 & & 1565 &    \\
    $R^2$   & 0.682 &  &  & &  &  \\
\bottomrule
\end{tabular}}

==> tables/table4.tex <==
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\toprule
      & \multicolumn{2}{c}{Circuitous and T-intersections} & \multicolumn{2}{c}{Low Density Deformed Grid} & \multicolumn{2}{c}{Medium Density Deformed Grid} & \multicolumn{2}{c}{Modernist superblocks} & \multicolumn{2}{c}{Dead Ends} & \multicolumn{2}{c}{High density grid} \\
     \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13} & 
     \multicolumn{1}{c}{coef.}  & \multicolumn{1}{c}{beta} & \multicolumn{1}{c}{coef.} & \multicolumn{1}{c}{beta} & \multicolumn{1}{c}{coef.} & \multicolumn{1}{c}{beta} & \multicolumn{1}{c}{coef.} & \multicolumn{1}{c}{beta} & \multicolumn{1}{c}{coef.} & \multicolumn{1}{c}{beta} & \multicolumn{1}{c}{coef.} & \multicolumn{1}{c}{beta} \\
\midrule
      K average (log) &   0.830 &  0.040   & -4.790*** &  -0.448   &  0.304 & -0.830 & -1.864*** & -0.764 &  -0.448 & -0.184 &   -3.131*** & -0.872    \\
            & (0.824)  & & (2.290)  & & (1.083)  & & (1.256)  & & (0.977)  & & (1.313) & \\
  Straightness & -13.164*** & -0.171 & -11.870* &  -0.071 &  -11.437*** &  -0.564   & -3.540 &  2.372   & -5.363* & 1.052 & 0.435 & 2.814 \\
  & (3.513) & & (12.522) & & (4.401) & & (5.625) & & (3.926) & & (4.205) & \\
 Intersection density &  -0.004* &  -0.311 & 0.000 & -0.041 &  0.0021 &  -0.123   & -0.001 &  -0.131   &   -0.024*** &  -0.605   &   -0.001 &  -0.211   \\
 & (0.002) & & (0.002) & & (0.003) & & (0.002) & & (0.004) & & (0.002) & \\
 Length per capita (log) &   0.835*** & 0.376 & 0.425 & 0.340 & 0.426* & 0.295 &  0.683*** & 0.341 &   3.365*** &  1.066   &   0.861*** &  0.381 \\
 & (0.166) & & (0.484) & & (0.391) & & (0.303) & & (0.422) & & (0.256) & \\
    Built up area (log) &   0.639*** & 0.755 &  1.083*** &  0.804 &  0.305*** & 0.343 &  0.680*** & 0.812 &   0.239** & 0.342 &  0.504*** & 0.622 \\
    & (0.066) & & (0.217) & & (0.114) & & (0.091) & & (0.090) & & (0.111) & \\
    Open space (log) &  -0.273 &  -0.051   &  5.812*** & 2.125 &  0.534*** & 0.766 &  0.947*** & 1.286 &  0.425*** & 0.381* &  1.007*** & 1.248 \\
    & (0.200) & & (1.722) & & (0.373) & & (0.325) & & (0.212) & & (0.537) & \\
       Population density (log) &   0.490*** & 0.253 &  -0.294 & -0.483 &   -0.445** & -1.922 &  0.291* &  -0.273 &  2.655*** &  3.199   &  0.309*** &  -0.189 \\
       & (0.151) & & (0.657) & & (0.343) & & (0.290) & & (0.429) & & (0.243) & \\
   GDP per capita (log) &   0.404*** & 0.259 &  0.007 &  0.019 &  0.517*** & 0.509 & 0.326*** & 0.067 &  0.157* &  -0.160   &  0.439*** & 0.327 \\
   & (0.080) & & (0.088) & & (0.114) & & (0.099) & & (0.097) & & (0.148) & \\
Night light per capita (log) &   0.349*** & 0.204 &  0.474*** &  0.308   & 0.107* & -0.419 &  0.493*** & 0.613 &   0.042 & -0.320 &   0.514*** &  0.620 \\
& (0.079) & & (0.157) & & (0.117) & & (0.100) & & (0.111) & & (0.139) & \\
  Grade median & -17.565*** & -0.131* & -11.780 &  -0.112   & -6.137* & -0.020 &  0.750 &   0.074  & -5.324 &  -0.073   &  -10.359** &  -0.085 \\
  & (7.242) & & (8.397) & & (8.310) & & (8.344) & & (8.280) & & (9.098) & \\
\midrule
    $n$ &  1692 &  &  665 & & 2362 & &  1244 &  & 1759 &   & 231  &   \\
    $R^2$   & 0.661 &  &  & &  & &  &  & &  &  &  \\
\bottomrule
\end{tabular}}
